Improved Online Contention Resolution for Matchings and Applications to the Gig Economy

Motivated by applications in the gig economy, we study approximation algorithms for a \emph{sequential pricing problem}. The input is a bipartite graph $G=(I,J,E)$ between individuals $I$ and jobs $J$. The platform has a value of $v_j$ for matching job $j$ to an individual worker. In order to find a matching, the platform can consider the edges $(i j) \in E$ in any order and make a one-time take-it-or-leave-it offer of a price $\pi_{ij} = w$ of its choosing to $i$ for completing $j$. The worker accepts the offer with a known probability $ p_{ijw} $; in this case the job and the worker are irrevocably matched. What is the best way to make offers to maximize revenue and/or social welfare? The optimal algorithm is known to be NP-hard to compute (even if there is only a single job). With this in mind, we design efficient approximations to the optimal policy via a new Random-Order Online Contention Resolution Scheme (RO-OCRS) for matching. Our main result is a 0.456-balanced RO-OCRS in bipartite graphs and a 0.45-balanced RO-OCRS in general graphs. These algorithms improve on the recent bound of $\frac{1}{2}(1-e^{-2})\approx 0.432$ of [BGMS21], and improve on the best known lower bounds for the correlation gap of matching, despite applying to a significantly more restrictive setting. As a consequence of our OCRS results, we obtain a $0.456$-approximate algorithm for the sequential pricing problem. We further extend our results to settings where workers can only be contacted a limited number of times, and show how to achieve improved results for this problem, via improved algorithms for the well-studied stochastic probing problem.

==> Improved Online Contention Resolution for Matchings and Applications to the Gig Economy (ArXiv)/olderMaterial.tex <==
\section{Random-order based algorithm}\label{sec: random-order}

\begin{comment}
\paragraph{The LP.}
\begin{align}
    \max & \sum_{e,w} x_{ew}\cdot p_{ew}\cdot w \\
    \textrm{s.t.} & \sum_{w} x_{ew}  \leq 1 \qquad \qquad\qquad\, \forall e \label{eqn:single-probe} \\
    & \sum_{e\ni v}\sum_{w} x_{ew}\cdot p_{ew}  \leq 1  \qquad \,\, \forall v \label{eqn:single-success} \\
    & x_{ew}  \geq 0 \qquad \qquad \qquad\qquad \forall e,w. \label{eqn:positivity}
\end{align}

\begin{align}
    \max & \sum_{i,j,w} x_{ijw}\cdot p_{ijw}\cdot w \\
    & \sum_{w} x_{ijw}  \leq 1 \qquad \qquad\,\, \forall i,j \label{eqn:single-probe} \\
    & \sum_{j,w} x_{ijw}\cdot p_{ijw}  \leq 1  \qquad \forall i \label{eqn:single-success-i} \\
    & \sum_{i,w} x_{ijw}\cdot p_{ijw} \leq 1 \qquad \forall j \label{eqn:single-success-j} \\
    &x_{ijw}  \geq 0 \qquad \qquad \qquad\,\, \forall i,j,w. \label{eqn:positivity}
\end{align}
\end{comment}

Denote by $\alpha_{e} \triangleq \sum_w x_{e,w}\cdot p_{e,w}$, and say an edge $e$ is \emph{free} at its arrival if neither of its endpoints is already matched.
Consider the following algorithm. (Here, $s$ is short for down-\underline{\textbf{s}}ampling.)

\begin{algorithm}
    \begin{algorithmic}[1]
        \For{each edge $e$, \textbf{in random order,}}
            \State draw $w$ from the multinomial distribution $\{x_{e,w}\}_w$
            \If{$e$ is free and probe $(e,w)$ successful}
    		        \State sell $e$ at price $w$, \textbf{with probability} $s(\alpha_{e})$
	        \EndIf
	    \EndFor
	\end{algorithmic}
    \caption{}
    \label{alg:main}
\end{algorithm}

\subsection{Warm-up: $1/3$-approximate algorithm}
In this section we consider the simplest instantiation of \Cref{alg:main}: the one with no down-sampling, i.e., with $s(x)=1$. The following lemma immediately implies that this algorithm is $1/3$ approximate.
\begin{lem}\label{lem:warmup}
    Denote by $\Pr[e \textrm{ free}]$ the probability that $e=(i,j)$ is free when inspected. Then, 
    $$\Pr[e \textrm{ free}] \geq \frac{1}{3}.$$
\end{lem}
\begin{proof}
    We note that $e$ is free if for none of the edges $f\in (\delta(i)\cup \delta(j))\setminus \{e\}$ arriving before $e$ we draw a weight $w$ whose probe is successful for $f$. Therefore, we have
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f)\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f) \,\,dz \\
        & \geq \int_0^1 (1-z\cdot (1-\alpha_e))^2\,\,dz & \textrm{Eqn. \eqref{eqn:single-success} + \Cref{fact:warmup}} \\
        & \geq \int_0^1 (1-z)^2\,\,dz & \textrm{Eqn. \eqref{eqn:positivity}} \\
        & = \frac{1}{3}. & \qedhere
    \end{align*}
\end{proof}

\begin{fact}\label{fact:warmup}
    Let $a_1,a_2,\dots,a_n\geq 0$. Then $\prod_{i=1}^n (1-a_i) \geq 1-\sum_{i=1}^n a_i$. 
\end{fact}
We defer a proof \Cref{fact:warmup}, which is easily proven by induction, as we will use (and prove) a stronger version of the above in the following section.

\subsection{Stronger Bound}

\paragraph{A bit of intuition:} We revisit the proof of \Cref{lem:warmup}, focusing on the latter two inequalities, and note when these are loose:\footnote{The argument behind the first inequality seems tricky to tighten.} the third inequality is trivially loose when $\alpha_e$ is bounded away from zero. 
Therefore, for edges $e$ with $\alpha_e \geq \theta$ for some large enough $\theta>0$, we can afford to down-sample $e$ with some probability $c:=c(\alpha_e)<1$, and still have $\Pr[e \textrm{ free}] \geq 1/3+\epsilon$ for some $\epsilon>0$.
This down-sampling proves useful when we consider edges $e$ with $\alpha_e\approx 0$, since one of the following must hold for such edge $e=(i,j)$: some edge $f\in (\delta(i)\cup \delta(j))\setminus\{e\}$ has $\alpha_f \geq \theta$, in which case the factor $1-z\cdot \alpha_f$ should be replaced with the (larger) term $1-z\cdot c\cdot \alpha_f$.
If, on the other hand, all edges $f\in (\delta(i)\cup \delta(j))\setminus\{e\}$ have $\alpha_f < \theta$, then the use of \Cref{fact:warmup} is loose, since this inequality is only tight when at most one $i$ has $a_i\neq 0$. In either case, the second inequality in the proof of \Cref{lem:warmup} is loose, and again we have $\Pr[e \textrm{ free}] \geq \frac{1}{3}+\epsilon$.


In what follows we will generalize this intuition and provide a tighter bound. We start with a simple technical fact, generalizing \Cref{fact:warmup}.\footnote{This must be known, right? Does this follow from some basic inequality? What's a source to cite here?}

\begin{fact}\label{fact:generalized}
    Let $a_1,a_2,\dots,a_n \in [0,\theta)$, and let $A_j:=\sum_{i=1}^j a_i$ for all $j\in [n]$. Then, 
    \begin{align}
    \prod_{i=1}^n (1-a_i)\geq (1-\theta)^{\lfloor A_n/\theta\rfloor} \cdot (1-(A_n-\lfloor A_n/\theta \rfloor \cdot \theta)).\label{ineq:general-fact}
    \end{align}
\end{fact}
\begin{proof}
    We prove the above by induction on $n\geq 1$. The first interesting case is clearly $n=2$,  which we later make use of for the inductive step.
    If $a_1+a_2 < \theta$, then \eqref{ineq:general-fact} reduces to $(1-a_1)(1-a_2) \geq (1-a_1-a_2)$, which holds since $a_1,a_2\geq 0$ implies $a_1\cdot a_2\geq 0$.
    If, however, $a_1+a_2\in [\theta,2\theta)$, then $$(1-a_1)(1-a_2) = 1-a_1-a_2+a_1\cdot a_2 \geq 1-a_1-a_2+\theta\cdot (a_1+a_2-\theta) = (1-\theta) (1-A_2-\theta),$$ 
    where the inequality follows from $a_1\cdot a_2\geq \theta\cdot (a_1+a_2-\theta)$, since the term $a_1\cdot a_2 - \theta\cdot (a_1+a_2-\theta)$ is monotone increasing in both $a_1$ and $a_2$, and thus the minimum of this latter expression subject to $a_1+a_2\geq \theta$ is zero.
    Now, suppose we have proven the above for $n-1$. Therefore,
    $\prod_{i=1}^{n-1} (1-a_i)\geq (1-\theta)^{\lfloor A_{n-1}/\theta\rfloor} \cdot (1-A_{n-1}-\lfloor A_{n-1}/\theta \rfloor\cdot \theta).$ 
    By the proof of the $n=2$ case applied to $a'_1 = A_{n-1} - \lfloor A_{n-1}/\theta\rfloor\cdot \theta \geq 0$ and $a'_2 = a_n \geq 0$, 
    we have that 
    $$(1-A_{n-1}-\lfloor A_{n-1}/\theta \rfloor\cdot \theta)(1-a_n)\geq (1-\theta)^{\lfloor (a'_1+a'_2)/\theta\rfloor}(1-(a'_1+a'_2-\lfloor (a'_1+a'_2)/\theta\rfloor\cdot \theta)).$$
    Combining with the inductive hypothesis, since $a'_1+a'_2-\lfloor (a'_1+a'_2)/\theta\rfloor\cdot \theta = A_n - \lfloor A_n/\theta\rfloor\cdot \theta$, 
    the desired bound follows. 
\end{proof}

\subsubsection{A concrete improvement}
Consider the following simple down-sampling, with $\theta=1/4$ and $c =\frac{9}{10}$ (neither optimized yet):
\begin{align}
    s(\alpha) = \begin{cases}
    1 & \alpha < \theta \\
    c & \alpha \geq \theta.
    \end{cases}
\end{align}

\begin{lem}\label{lem:concrete}
    For any edge $e$, we have that $s(\alpha_e)\cdot \Pr[e \textrm{ free}]$ is at least
    \begin{align*}
         \min\left\{c\cdot \int_0^1 (1-z\cdot (1-\theta)^2))\,\,dz,\,\, \int_0^1 (1-z)(1-z\cdot (1-c\cdot \theta)) \,\,dz, \,\, \int_0^1 (1-\theta)^{\lfloor 2z/\theta \rfloor}(1-(2z-\lfloor 2z/\theta \rfloor\cdot \theta))\right\}.
    \end{align*}
    For $c=4/5$ and $\theta=1/4$, the above is at least $0.3375$.
\end{lem}
\begin{proof}
    Let $e=(i,j)$.
    First, suppose $\alpha_e \geq \theta$. Similarly to the proof of \Cref{lem:warmup}, we have that
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))) \,\,dz \\
        & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f)\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f) \,\,dz & s(\alpha_f)\leq 1\\
        & \geq \int_0^1 (1-z\cdot (1-\alpha_e))^2\,\,dz & \textrm{Cons. \eqref{eqn:single-success} + \Cref{fact:warmup}} \\
        & \geq \int_0^1 (1-z\cdot(1-\theta))^2\,\,dz & \alpha_e\geq \theta 
        \\ & = \frac{7}{16}. & \theta= 1/4
    \end{align*}
    Consequently, we have $s(\alpha_e)\cdot \Pr[e \textrm{ free}] \geq c\cdot \frac{7}{16} = \frac{63}{160} = 0.39375$.
    
    Next, suppose $\alpha_e \leq \theta$. For vertex $v$, let $A_v := \sum_{f\in \delta(v): \alpha_f\geq \theta} \alpha_f$.
    If $A_i+A_j\geq \theta$, there is some $f^*\in \delta(i)\cup \delta(j)$ with $\alpha_{f^*}\geq \theta$, and we have that 
   \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))) \,\,dz \\
        & \geq \int_{0}^1 (1-z\cdot (1-\alpha_e))(1-z\cdot (1-\alpha_e - (1-c)\cdot \alpha_{f^*})) \,\,dz & \textrm{\Cref{fact:warmup}, \, Cons. \eqref{eqn:single-success}}
        \\
        & \geq \int_0^1 (1-z)(1-z\cdot (1-(1-c)\cdot \theta)) \,\,dz. & \textrm{Cons. \eqref{eqn:positivity}}, \,\alpha_{f^*}\geq \theta \\
        & = \int_0^1 (1-z)(1-z\cdot (1-1/40)) \,\,dz. & c=9/10, \theta=1/4\\
        & = \frac{27}{80} = 0.3375.
    \end{align*}
    Now, suppose $A_i+A_j < \theta$. 
    Then, we have that $A_i,A_j < \theta$. 
    Let $B_v:=\sum_{f\in \delta(v)\setminus\{e\}: \alpha_f < \theta} \alpha_f$. By \eqref{eqn:single-success}, we have that $A_i+B_i\leq 1-\alpha_e$ and $A_j+B_j\leq 1-\alpha_e$. Since $\alpha_e < \theta$ and $A_i,A_j<\theta$, we have that $1-\alpha_e - A_i > 1-2\theta$. Therefore, by \Cref{fact:generalized}, we have the following.
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f)\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f) \,\,dz \\
        & \geq \int_{0}^1 (1-\theta)^{\lfloor z\cdot (B_i+B_j)/\theta\rfloor}(1-(z(B_i+B_j)-\lfloor z(B_i+B_j)/\theta\rfloor\cdot \theta))
         \,\,dz & \\
        & \geq \int_0^1 (1-\theta)^{\lfloor 2z/\theta \rfloor}(1-(2z-\lfloor 2z/\theta \rfloor\cdot \theta))\,\, dz & B_i,B_j\leq 1-\alpha_e \leq 1\\
        & \approx 0.393. & \theta=1/4.
    \end{align*}
\end{proof}

\subsection{Refining the analysis}

\paragraph{Intuition.} The analysis in the proof of \Cref{lem:concrete} was fairly loose when considering an edge $e=(i,j)$ with $\alpha_e<\theta$ and any number of edges $f\in \delta(i)\cup \delta(j)$ with $\alpha_f\geq \theta$. In particular, it made no use of \Cref{fact:generalized} when accounting for edges $f\in \delta(i)\cup \delta(j)$ other than $f^*$.
Essentially, a better bound would follow by combining both cases considered for edge $e$ with $\alpha_e < \theta$.

We now revisit and refine the proof of \Cref{lem:concrete}.
By facts \ref{fact:warmup} and \ref{fact:generalized}, we have that
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))) \,\,dz \\
        & \geq \int_0^1 (1-z\cdot c\cdot A_i) (1-z\cdot c\cdot A_j) 
        (1-\theta)^{\lfloor(B_i+B_j)/\theta \rfloor} (1-z\cdot (B_i+B_j-\lfloor(B_i+B_j)/\theta \rfloor\cdot \theta)) \,\, dz
    \end{align*}

    \paragraph{Limits to step functions $s(\cdot)$.}
    With the step function kind of down-sampling function $s(\cdot)$, the best we could hope to get here is $\Pr[e \textrm{ free}] \geq \int_0^1 (1-z\cdot c)^2\,\,dz$, which, for the above choice of $c=9/10$ comes out to $0.37.$
    However, here, too, for this argument to be tight for $e=(i,j)$, we need $\alpha_e\approx 0$ and $i,j$ both to have a single edge $f$ each with $\alpha_f \approx 1$. But in this case such an edge $f$ can be down-sampled much more aggressively, since the probability such an edge $f$ is free is basically one.
    Generally, it seems reasonable to have $s(\alpha_e)$ be a (smoother) monotone increasing function of $\alpha_e$, which behaves nicely with the integral forms obtained.
    


    
\section{OCRS-Based Algorithm}   

\begin{algorithm}\label{alg:OCRS}
    \begin{algorithmic}[1]
        \For{each edge $e$ and weight $w$, \textbf{in arbitrary order,}}
            \If{$e$ is free and not probed yet}
    		        \State probe $e$ at price $w$, \textbf{with probability} $\frac{c\cdot x_{e,w}}{\Pr[e \textrm{ free \& not probed}]}$
	        \EndIf
	    \EndFor
	\end{algorithmic}
    \caption{}
    \label{alg:main}
\end{algorithm}

Our goal is to find the maximum $c$ such that the above algorithm is well-defined. Therefore, for a specific $c$, we have to show that line 3 of the algorithm is well-defined, in other words, we need to show that $c\cdot x_{e,w} \leq \Pr[e \textrm{ free \& not probed}]$. For $e=(u,v)$ we have that

\begin{align*}
    \Pr[e \textrm{ free \& not probed}] \geq 1 - \Pr[u \textrm{ matched}] - \Pr[v \textrm{ matched}] - \Pr[e \textrm{ probed}]
\end{align*}
    
By Eqn.\eqref{eqn:single-success} and the fact that the algorithm downsample the probabilities $x_{e,w}$ by a factor $c$, we have that $\Pr[v \textrm{ matched}] \leq c$ at anytime during the algorithm. Moreover, with the same argument and using Eqn.\eqref{eqn:single-probe}, we have that $\Pr[e \textrm{ probed}] \leq c\cdot(1-x_{e,w})$. Hence, we have that

\begin{align*}
    \Pr[e \textrm{ free \& not probed}] &\geq 1 - \Pr[u \textrm{ matched}] - \Pr[v \textrm{ matched}] - \Pr[e \textrm{ probed}]
    \\
    & \geq 1 - c - c - c\cdot(1 - x_{e,w})
    \\
    & \geq 1 - 3c + c\cdot x_{e,w}
\end{align*}

If we choose $c=1/3$, then 

\begin{align*}
\Pr[e \textrm{ free \& not probed}] \geq c\cdot x_{e,w}
\end{align*}

Therefore, Algorithm \ref{alg:OCRS} is well-defined. Since we can run this algorithm on any arbitrary ordering of edges and weights, it will be incentive-compatible if we probe according to the increasing order of weights.

\subsection{Next Steps}
\begin{enumerate}
    \item \textbf{Witness:} We can use witnesses to strengthen the union bound to get $c=0.341$.
\end{enumerate}

==> olderMaterial.tex <==
\section{Random-order based algorithm}\label{sec: random-order}

\begin{comment}
\paragraph{The LP.}
\begin{align}
    \max & \sum_{e,w} x_{ew}\cdot p_{ew}\cdot w \\
    \textrm{s.t.} & \sum_{w} x_{ew}  \leq 1 \qquad \qquad\qquad\, \forall e \label{eqn:single-probe} \\
    & \sum_{e\ni v}\sum_{w} x_{ew}\cdot p_{ew}  \leq 1  \qquad \,\, \forall v \label{eqn:single-success} \\
    & x_{ew}  \geq 0 \qquad \qquad \qquad\qquad \forall e,w. \label{eqn:positivity}
\end{align}

\begin{align}
    \max & \sum_{i,j,w} x_{ijw}\cdot p_{ijw}\cdot w \\
    & \sum_{w} x_{ijw}  \leq 1 \qquad \qquad\,\, \forall i,j \label{eqn:single-probe} \\
    & \sum_{j,w} x_{ijw}\cdot p_{ijw}  \leq 1  \qquad \forall i \label{eqn:single-success-i} \\
    & \sum_{i,w} x_{ijw}\cdot p_{ijw} \leq 1 \qquad \forall j \label{eqn:single-success-j} \\
    &x_{ijw}  \geq 0 \qquad \qquad \qquad\,\, \forall i,j,w. \label{eqn:positivity}
\end{align}
\end{comment}

Denote by $\alpha_{e} \triangleq \sum_w x_{e,w}\cdot p_{e,w}$, and say an edge $e$ is \emph{free} at its arrival if neither of its endpoints is already matched.
Consider the following algorithm. (Here, $s$ is short for down-\underline{\textbf{s}}ampling.)

\begin{algorithm}
    \begin{algorithmic}[1]
        \For{each edge $e$, \textbf{in random order,}}
            \State draw $w$ from the multinomial distribution $\{x_{e,w}\}_w$
            \If{$e$ is free and probe $(e,w)$ successful}
    		        \State sell $e$ at price $w$, \textbf{with probability} $s(\alpha_{e})$
	        \EndIf
	    \EndFor
	\end{algorithmic}
    \caption{}
    \label{alg:main}
\end{algorithm}

\subsection{Warm-up: $1/3$-approximate algorithm}
In this section we consider the simplest instantiation of \Cref{alg:main}: the one with no down-sampling, i.e., with $s(x)=1$. The following lemma immediately implies that this algorithm is $1/3$ approximate.
\begin{lem}\label{lem:warmup}
    Denote by $\Pr[e \textrm{ free}]$ the probability that $e=(i,j)$ is free when inspected. Then, 
    $$\Pr[e \textrm{ free}] \geq \frac{1}{3}.$$
\end{lem}
\begin{proof}
    We note that $e$ is free if for none of the edges $f\in (\delta(i)\cup \delta(j))\setminus \{e\}$ arriving before $e$ we draw a weight $w$ whose probe is successful for $f$. Therefore, we have
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f)\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f) \,\,dz \\
        & \geq \int_0^1 (1-z\cdot (1-\alpha_e))^2\,\,dz & \textrm{Eqn. \eqref{eqn:single-success} + \Cref{fact:warmup}} \\
        & \geq \int_0^1 (1-z)^2\,\,dz & \textrm{Eqn. \eqref{eqn:positivity}} \\
        & = \frac{1}{3}. & \qedhere
    \end{align*}
\end{proof}

\begin{fact}\label{fact:warmup}
    Let $a_1,a_2,\dots,a_n\geq 0$. Then $\prod_{i=1}^n (1-a_i) \geq 1-\sum_{i=1}^n a_i$. 
\end{fact}
We defer a proof \Cref{fact:warmup}, which is easily proven by induction, as we will use (and prove) a stronger version of the above in the following section.

\subsection{Stronger Bound}

\paragraph{A bit of intuition:} We revisit the proof of \Cref{lem:warmup}, focusing on the latter two inequalities, and note when these are loose:\footnote{The argument behind the first inequality seems tricky to tighten.} the third inequality is trivially loose when $\alpha_e$ is bounded away from zero. 
Therefore, for edges $e$ with $\alpha_e \geq \theta$ for some large enough $\theta>0$, we can afford to down-sample $e$ with some probability $c:=c(\alpha_e)<1$, and still have $\Pr[e \textrm{ free}] \geq 1/3+\epsilon$ for some $\epsilon>0$.
This down-sampling proves useful when we consider edges $e$ with $\alpha_e\approx 0$, since one of the following must hold for such edge $e=(i,j)$: some edge $f\in (\delta(i)\cup \delta(j))\setminus\{e\}$ has $\alpha_f \geq \theta$, in which case the factor $1-z\cdot \alpha_f$ should be replaced with the (larger) term $1-z\cdot c\cdot \alpha_f$.
If, on the other hand, all edges $f\in (\delta(i)\cup \delta(j))\setminus\{e\}$ have $\alpha_f < \theta$, then the use of \Cref{fact:warmup} is loose, since this inequality is only tight when at most one $i$ has $a_i\neq 0$. In either case, the second inequality in the proof of \Cref{lem:warmup} is loose, and again we have $\Pr[e \textrm{ free}] \geq \frac{1}{3}+\epsilon$.


In what follows we will generalize this intuition and provide a tighter bound. We start with a simple technical fact, generalizing \Cref{fact:warmup}.\footnote{This must be known, right? Does this follow from some basic inequality? What's a source to cite here?}

\begin{fact}\label{fact:generalized}
    Let $a_1,a_2,\dots,a_n \in [0,\theta)$, and let $A_j:=\sum_{i=1}^j a_i$ for all $j\in [n]$. Then, 
    \begin{align}
    \prod_{i=1}^n (1-a_i)\geq (1-\theta)^{\lfloor A_n/\theta\rfloor} \cdot (1-(A_n-\lfloor A_n/\theta \rfloor \cdot \theta)).\label{ineq:general-fact}
    \end{align}
\end{fact}
\begin{proof}
    We prove the above by induction on $n\geq 1$. The first interesting case is clearly $n=2$,  which we later make use of for the inductive step.
    If $a_1+a_2 < \theta$, then \eqref{ineq:general-fact} reduces to $(1-a_1)(1-a_2) \geq (1-a_1-a_2)$, which holds since $a_1,a_2\geq 0$ implies $a_1\cdot a_2\geq 0$.
    If, however, $a_1+a_2\in [\theta,2\theta)$, then $$(1-a_1)(1-a_2) = 1-a_1-a_2+a_1\cdot a_2 \geq 1-a_1-a_2+\theta\cdot (a_1+a_2-\theta) = (1-\theta) (1-A_2-\theta),$$ 
    where the inequality follows from $a_1\cdot a_2\geq \theta\cdot (a_1+a_2-\theta)$, since the term $a_1\cdot a_2 - \theta\cdot (a_1+a_2-\theta)$ is monotone increasing in both $a_1$ and $a_2$, and thus the minimum of this latter expression subject to $a_1+a_2\geq \theta$ is zero.
    Now, suppose we have proven the above for $n-1$. Therefore,
    $\prod_{i=1}^{n-1} (1-a_i)\geq (1-\theta)^{\lfloor A_{n-1}/\theta\rfloor} \cdot (1-A_{n-1}-\lfloor A_{n-1}/\theta \rfloor\cdot \theta).$ 
    By the proof of the $n=2$ case applied to $a'_1 = A_{n-1} - \lfloor A_{n-1}/\theta\rfloor\cdot \theta \geq 0$ and $a'_2 = a_n \geq 0$, 
    we have that 
    $$(1-A_{n-1}-\lfloor A_{n-1}/\theta \rfloor\cdot \theta)(1-a_n)\geq (1-\theta)^{\lfloor (a'_1+a'_2)/\theta\rfloor}(1-(a'_1+a'_2-\lfloor (a'_1+a'_2)/\theta\rfloor\cdot \theta)).$$
    Combining with the inductive hypothesis, since $a'_1+a'_2-\lfloor (a'_1+a'_2)/\theta\rfloor\cdot \theta = A_n - \lfloor A_n/\theta\rfloor\cdot \theta$, 
    the desired bound follows. 
\end{proof}

\subsubsection{A concrete improvement}
Consider the following simple down-sampling, with $\theta=1/4$ and $c =\frac{9}{10}$ (neither optimized yet):
\begin{align}
    s(\alpha) = \begin{cases}
    1 & \alpha < \theta \\
    c & \alpha \geq \theta.
    \end{cases}
\end{align}

\begin{lem}\label{lem:concrete}
    For any edge $e$, we have that $s(\alpha_e)\cdot \Pr[e \textrm{ free}]$ is at least
    \begin{align*}
         \min\left\{c\cdot \int_0^1 (1-z\cdot (1-\theta)^2))\,\,dz,\,\, \int_0^1 (1-z)(1-z\cdot (1-c\cdot \theta)) \,\,dz, \,\, \int_0^1 (1-\theta)^{\lfloor 2z/\theta \rfloor}(1-(2z-\lfloor 2z/\theta \rfloor\cdot \theta))\right\}.
    \end{align*}
    For $c=4/5$ and $\theta=1/4$, the above is at least $0.3375$.
\end{lem}
\begin{proof}
    Let $e=(i,j)$.
    First, suppose $\alpha_e \geq \theta$. Similarly to the proof of \Cref{lem:warmup}, we have that
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))) \,\,dz \\
        & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f)\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f) \,\,dz & s(\alpha_f)\leq 1\\
        & \geq \int_0^1 (1-z\cdot (1-\alpha_e))^2\,\,dz & \textrm{Cons. \eqref{eqn:single-success} + \Cref{fact:warmup}} \\
        & \geq \int_0^1 (1-z\cdot(1-\theta))^2\,\,dz & \alpha_e\geq \theta 
        \\ & = \frac{7}{16}. & \theta= 1/4
    \end{align*}
    Consequently, we have $s(\alpha_e)\cdot \Pr[e \textrm{ free}] \geq c\cdot \frac{7}{16} = \frac{63}{160} = 0.39375$.
    
    Next, suppose $\alpha_e \leq \theta$. For vertex $v$, let $A_v := \sum_{f\in \delta(v): \alpha_f\geq \theta} \alpha_f$.
    If $A_i+A_j\geq \theta$, there is some $f^*\in \delta(i)\cup \delta(j)$ with $\alpha_{f^*}\geq \theta$, and we have that 
   \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))) \,\,dz \\
        & \geq \int_{0}^1 (1-z\cdot (1-\alpha_e))(1-z\cdot (1-\alpha_e - (1-c)\cdot \alpha_{f^*})) \,\,dz & \textrm{\Cref{fact:warmup}, \, Cons. \eqref{eqn:single-success}}
        \\
        & \geq \int_0^1 (1-z)(1-z\cdot (1-(1-c)\cdot \theta)) \,\,dz. & \textrm{Cons. \eqref{eqn:positivity}}, \,\alpha_{f^*}\geq \theta \\
        & = \int_0^1 (1-z)(1-z\cdot (1-1/40)) \,\,dz. & c=9/10, \theta=1/4\\
        & = \frac{27}{80} = 0.3375.
    \end{align*}
    Now, suppose $A_i+A_j < \theta$. 
    Then, we have that $A_i,A_j < \theta$. 
    Let $B_v:=\sum_{f\in \delta(v)\setminus\{e\}: \alpha_f < \theta} \alpha_f$. By \eqref{eqn:single-success}, we have that $A_i+B_i\leq 1-\alpha_e$ and $A_j+B_j\leq 1-\alpha_e$. Since $\alpha_e < \theta$ and $A_i,A_j<\theta$, we have that $1-\alpha_e - A_i > 1-2\theta$. Therefore, by \Cref{fact:generalized}, we have the following.
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f)\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f) \,\,dz \\
        & \geq \int_{0}^1 (1-\theta)^{\lfloor z\cdot (B_i+B_j)/\theta\rfloor}(1-(z(B_i+B_j)-\lfloor z(B_i+B_j)/\theta\rfloor\cdot \theta))
         \,\,dz & \\
        & \geq \int_0^1 (1-\theta)^{\lfloor 2z/\theta \rfloor}(1-(2z-\lfloor 2z/\theta \rfloor\cdot \theta))\,\, dz & B_i,B_j\leq 1-\alpha_e \leq 1\\
        & \approx 0.393. & \theta=1/4.
    \end{align*}
\end{proof}

\subsection{Refining the analysis}

\paragraph{Intuition.} The analysis in the proof of \Cref{lem:concrete} was fairly loose when considering an edge $e=(i,j)$ with $\alpha_e<\theta$ and any number of edges $f\in \delta(i)\cup \delta(j)$ with $\alpha_f\geq \theta$. In particular, it made no use of \Cref{fact:generalized} when accounting for edges $f\in \delta(i)\cup \delta(j)$ other than $f^*$.
Essentially, a better bound would follow by combining both cases considered for edge $e$ with $\alpha_e < \theta$.

We now revisit and refine the proof of \Cref{lem:concrete}.
By facts \ref{fact:warmup} and \ref{fact:generalized}, we have that
    \begin{align*}
        \Pr[e \textrm{ free}] & \geq \int_{0}^1 \prod_{f\in \delta(i)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))\cdot \prod_{f\in \delta(j)\setminus \{e\}}(1-z\cdot \alpha_f\cdot s(\alpha_f))) \,\,dz \\
        & \geq \int_0^1 (1-z\cdot c\cdot A_i) (1-z\cdot c\cdot A_j) 
        (1-\theta)^{\lfloor(B_i+B_j)/\theta \rfloor} (1-z\cdot (B_i+B_j-\lfloor(B_i+B_j)/\theta \rfloor\cdot \theta)) \,\, dz
    \end{align*}

    \paragraph{Limits to step functions $s(\cdot)$.}
    With the step function kind of down-sampling function $s(\cdot)$, the best we could hope to get here is $\Pr[e \textrm{ free}] \geq \int_0^1 (1-z\cdot c)^2\,\,dz$, which, for the above choice of $c=9/10$ comes out to $0.37.$
    However, here, too, for this argument to be tight for $e=(i,j)$, we need $\alpha_e\approx 0$ and $i,j$ both to have a single edge $f$ each with $\alpha_f \approx 1$. But in this case such an edge $f$ can be down-sampled much more aggressively, since the probability such an edge $f$ is free is basically one.
    Generally, it seems reasonable to have $s(\alpha_e)$ be a (smoother) monotone increasing function of $\alpha_e$, which behaves nicely with the integral forms obtained.
    


    
\section{OCRS-Based Algorithm}   

\begin{algorithm}\label{alg:OCRS}
    \begin{algorithmic}[1]
        \For{each edge $e$ and weight $w$, \textbf{in arbitrary order,}}
            \If{$e$ is free and not probed yet}
    		        \State probe $e$ at price $w$, \textbf{with probability} $\frac{c\cdot x_{e,w}}{\Pr[e \textrm{ free \& not probed}]}$
	        \EndIf
	    \EndFor
	\end{algorithmic}
    \caption{}
    \label{alg:main}
\end{algorithm}

Our goal is to find the maximum $c$ such that the above algorithm is well-defined. Therefore, for a specific $c$, we have to show that line 3 of the algorithm is well-defined, in other words, we need to show that $c\cdot x_{e,w} \leq \Pr[e \textrm{ free \& not probed}]$. For $e=(u,v)$ we have that

\begin{align*}
    \Pr[e \textrm{ free \& not probed}] \geq 1 - \Pr[u \textrm{ matched}] - \Pr[v \textrm{ matched}] - \Pr[e \textrm{ probed}]
\end{align*}
    
By Eqn.\eqref{eqn:single-success} and the fact that the algorithm downsample the probabilities $x_{e,w}$ by a factor $c$, we have that $\Pr[v \textrm{ matched}] \leq c$ at anytime during the algorithm. Moreover, with the same argument and using Eqn.\eqref{eqn:single-probe}, we have that $\Pr[e \textrm{ probed}] \leq c\cdot(1-x_{e,w})$. Hence, we have that

\begin{align*}
    \Pr[e \textrm{ free \& not probed}] &\geq 1 - \Pr[u \textrm{ matched}] - \Pr[v \textrm{ matched}] - \Pr[e \textrm{ probed}]
    \\
    & \geq 1 - c - c - c\cdot(1 - x_{e,w})
    \\
    & \geq 1 - 3c + c\cdot x_{e,w}
\end{align*}

If we choose $c=1/3$, then 

\begin{align*}
\Pr[e \textrm{ free \& not probed}] \geq c\cdot x_{e,w}
\end{align*}

Therefore, Algorithm \ref{alg:OCRS} is well-defined. Since we can run this algorithm on any arbitrary ordering of edges and weights, it will be incentive-compatible if we probe according to the increasing order of weights.

\subsection{Next Steps}
\begin{enumerate}
    \item \textbf{Witness:} We can use witnesses to strengthen the union bound to get $c=0.341$.
\end{enumerate}
